Compact Binary Coalescence Gravitational Wave Signals Counting and Separation

As next-generation gravitational-wave (GW) observatories approach unprecedented sensitivities, the need for robust methods to analyze increasingly complex, overlapping signals becomes ever more pressing. Existing matched-filtering approaches and deep-learning techniques can typically handle only one or two concurrent signals, offering limited adaptability to more varied and intricate superimposed waveforms. To overcome these constraints, we present the UnMixFormer, an attention-based architecture that not only identifies the unknown number of concurrent compact binary coalescence GW events but also disentangles their individual waveforms through a multi-decoder architecture, even when confronted with five overlapping signals. Our UnMixFormer is capable of capturing both short- and long-range dependencies by modeling them in a dual-path manner, while also enhancing periodic feature representation by incorporating Fourier Analysis Networks. Our approach adeptly processes binary black hole, binary neutron star, and neutron star-black hole systems over extended time series data (16,384 samples). When evaluating on synthetic data with signal-to-noise ratios (SNR) ranging from 10 to 50, our method achieves 99.89% counting accuracy, a mean overlap of 0.9831 between separated waveforms and templates, and robust generalization ability to waveforms with spin precession, orbital eccentricity, and higher modes, marking a substantial advance in the precision and versatility of GW data analysis.

==> myacro.tex <==
\usepackage{acro}
\acsetup{
barriers/use = true,
barriers/reset = true,
}

\DeclareAcroEnding{possessive}{'s}{'s}
\NewAcroCommand\acg{m}{\acropossessive\UseAcroTemplate{first}{#1}}
\NewAcroCommand\acsg{m}{\acropossessive\UseAcroTemplate{short}{#1}}
\NewAcroCommand\aclg{m}{\acropossessive\UseAcroTemplate{long}{#1}}
\NewAcroCommand\acfg{m}{%
    \acrofull
    \acropossessive
    \UseAcroTemplate{first}{#1}%
}
\NewAcroCommand\iacsg{m}{%
    \acroindefinite
    \acropossessive
    \UseAcroTemplate{short}{#1}%
}

\DeclareAcronym{AI}{
    short = AI,
    long  = artificial intelligence
}

\DeclareAcronym{AK}{
    short = AK,
    long  = analytic kludge
}
\DeclareAcronym{AAK}{
    short = AAK,
    long  = argumented analytic kludge
}
\DeclareAcronym{AUC}{
    short = AUC,
    long  = area under the curve
}
\DeclareAcronym{BH}{
    short = BH,
    long  = black hole
}
\DeclareAcronym{BHB}{
    short = BHB,
    long  = black hole binary,
    long-plural-form = black hole binaries
}
\DeclareAcronym{BBH}{
    short = BBH,
    long  = binary black hole
}

\DeclareAcronym{BNS}{
    short = BNS,
    long  = binary neutron star
}
\DeclareAcronym{CNN}{
    short = CNN,
    long  = convolutional neural network
}
\DeclareAcronym{CE}{
    short = CE,
    long  = Cosmic Explorer
}
\DeclareAcronym{CBC}{
    short = CBC,
    long  = compact binary coalescence
}
\DeclareAcronym{CBS}{
    short = CBS,
    long  = compact binary system
}

\DeclareAcronym{DECODE}{
    short = DECODE,
    long  = DECODE
}
\DeclareAcronym{DECIGO}{
    short = DECIGO,
    long  = DECi-hertz Interferometer Gravitational wave Observatory
}

\DeclareAcronym{DNN}{
    short = DNN,
    long  = deep neural network
}
\DeclareAcronym{ESA}{
    short = ESA,
    long  = European Space Agency
}
\DeclareAcronym{EMRI}{
    short = EMRI,
    long  = extreme-mass-ratio inspiral
}
\DeclareAcronym{ET}{
    short = ET,
    long  = Einstein Telescope
}
\DeclareAcronym{FPR}{
    short = FPR,
    long  = false positive rate
}
\DeclareAcronym{FAN}{
    short = FAN,
    long  = Fourier Analysis Network
}
\DeclareAcronym{GB}{
    short = GB,
    long  = galactic binary,
    long-plural-form = galactic binaries
}
\DeclareAcronym{GR}{
    short = GR,
    long  = general relativity
}
\DeclareAcronym{GW}{
    short = GW,
    long  = gravitational wave
}
\DeclareAcronym{LDC}{
    short = LDC,
    long  = LISA Data Challenge
}
\DeclareAcronym{LIGO}{
    short = LIGO,
    long  = \href{http://www.ligo.caltech.edu/}{Laser Interferemeter Gravitational Wave Observatory}
}
\DeclareAcronym{LISA}{
    short = LISA,
    long  = \href{https://www.lisamission.org/}{Laser Interferometer Space Antenna}
}

\DeclareAcronym{LSO}{
    short = LSO,
    long  = last stable orbit
}

\DeclareAcronym{MLP}{
    short = MLP,
    long  = multilayer perceptron
}

\DeclareAcronym{MBH}{
    short = MBH,
    long  = massive black hole
}
\DeclareAcronym{MBHB}{
    short = MBHB,
    long  = massive black hole binary,
    long-plural-form = massive black hole binaries
}

\DeclareAcronym{MCMC}{
    short = MCMC,
    long  = Markov-chain Monte Carlo
}
\DeclareAcronym{MLDC}{
    short = MLDC,
    long  = \href{http://astrogravs.nasa.gov/docs/mldc/}{Mock LISA Data Challenge}
}
\DeclareAcronym{NK}{
    short = NK,
    long  = numerical kludge
}
\DeclareAcronym{NSBH}{
    short = NS-BH,
    long  = neutron star-black hole
}
\DeclareAcronym{OMS}{
    short = OMS,
    long  = optical metrology system
}
\DeclareAcronym{PSD}{
    short = PSD,
    long  = power spectral density
}
\DeclareAcronym{ReLU}{
    short = ReLU,
    long  = rectified linear 
 unit
}

\DeclareAcronym{ROC}{
    short = ROC,
    long  = receiver operating characteristic
}
\DeclareAcronym{SGWB}{
    short = SGWB,
    long  = stochastic gravitational wave background
}
\DeclareAcronym{SMBH}{
    short = SMBH,
    long  = super-massive black hole
}
\DeclareAcronym{SNR}{
    short = SNR,
    long  = signal-to-noise ratio
}
\DeclareAcronym{SOBH}{
    short = SOBH,
    long  = stellar origin black hole binary
}
\DeclareAcronym{SSB}{
    short = SSB,
    long  = solar system barycenter
}
\DeclareAcronym{TCN}{
    short = TCN,
    long  = temporal convolutional network
}
\DeclareAcronym{TDI}{
    short = TDI,
    long  = time delay interferometry
}
\DeclareAcronym{TPR}{
    short = TPR,
    long  = true positive rate
}
\DeclareAcronym{t-SNE}{
    short = t-SNE,
    long  = t-distributed stochastic neighbor embedding
}
\DeclareAcronym{VGB}{
    short = VGB,
    long  = verification galactic binary,
    long-plural-form = verification galactic binaries
}
